Near Uniform Triangle Sampling Over Adjacency List Graph Streams

Triangle counting and sampling are two fundamental problems for streaming algorithms. Arguably, designing sampling algorithms is more challenging than their counting variants. It may be noted that triangle counting has received far greater attention in the literature than the sampling variant. In this work, we consider the problem of approximately sampling triangles in different models of streaming with the focus being on the adjacency list model. In this problem, the edges of a graph $G$ will arrive over a data stream. The goal is to design efficient streaming algorithms that can sample and output a triangle from a distribution, over the triangles in $G$, that is close to the uniform distribution over the triangles in $G$. The distance between distributions is measured in terms of $\ell_1$-distance. The main technical contribution of this paper is to design algorithms for this triangle sampling problem in the adjacency list model with the space complexities matching their counting variants. For the sake of completeness, we also show results on the vertex and edge arrival models.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> abstract.tex <==
% Counting and sampling are two fundamental problems in the field of sublinear algorithms. Over the last few years, there have been several new works with the goal of better understanding of the complexities of these problems. Although triangle counting has been extensively studied in the streaming literature, its sampling variant has not yet been explored. In this problem, the edges of a graph $G$ will arrive over a data stream and the goal is to output a distribution over the triangles of $G$ that is \emph{close} to the uniform distribution over the triangles. In this paper, we study this problem in three popular streaming models: namely in {\sc Vertex Arrival} model, {\sc Edge Arrival} model, and in {\sc Adjacency List} model. In all these three models, we present almost optimal algorithms for this problem. 
%
%
Counting and sampling are two fundamental problems in {\em sublinear algorithms}. Over the last few years, there have been several new works with the goal of better understanding the complexities of these problems. Although triangle counting has been extensively studied in the streaming literature, its sampling variant has not yet been explored. In this problem, the edges of a graph $G$ will arrive over a data stream. The goal is to output a sample from a distribution over the triangles in $G$ that is \emph{close} to the uniform distribution over the triangles in $G$, where the distance between distributions is measured in terms of $\ell_1$-distance. In this paper, we study this problem in three popular streaming models: namely in {\sc Edge Arrival} model, {\sc Vertex Arrival} model and {\sc Adjacency List} model. In all these three models, we present near optimal algorithms for this problem. 



==> al_algo_1pass.tex <==
\begin{algorithm}
\caption{Triangle Sampling in 1-pass \al Model}\label{alg:1passal} 
%Call {\sc Sample-Light-Triangle}. 

%Initiate a reservoir sampler $\mbox{{\sc RS}}$ such that $\mbox{{\sc RS}}$ keeps a set $\cF_1$ of $\tOh(m/\sqrt{T})$ edges. Also initiate a weighted reservoir  sampler {\sc WRS}.\ \label{algo:1passal_line1}

Set $p=100\log n/\eps^2 \sqrt{T}$ and  $\kappa= 10 {\log n}$.\ \label{algo:1passal_line2}

%// {We assume that $T$ is at least a polynomial in $\log n$ and $1/\eps$.} So, $p \in (0,1)$ .

Call \rouone and \routwo  in parallel.\ \label{algo:1passal_line3}



{\bf Process at the end of the stream:}


Call {\sc Sample-Light-Triangle}. Let $\Delta_L$ be the output.\ \label{algo:1passal_line4}

Call {\sc Sample-Heavy-Triangle}. Let $(\widehat{T}_H,\Delta_H)$ be the output.\ \label{algo:1passal_line5}

If either {\sc Sample-Light-Triangle} or {\sc Sample-Heavy-Triangle} report {\sc Fail}, then report {\sc Fail} and {\sc ABORT} the process.\ \label{algo:1passal_line6}


%If it reports {\sc Fail}, then report the same as the output. Otherwise, let $\widetilde{T_h}$ and $\Delta_h$ be its output.

\uIf{$\widehat{T}_H \leq \eps T/10 $}
{ 
\label{algo:1passal_line7}

Report $\Delta_L$ as the output.\ \label{algo:1passal_line8}

}

\uIf{$\widehat{T}_H \geq \left(1-\eps/10\right) T$} 
{

\label{algo:1passal_line9}

Report $\Delta_H$ as the output.\ \label{algo:1passal_line10}

}

Report $\Delta_H$ with probability $\widehat{T}_H/T$ and $\Delta_L$ with  probability $1-\widehat{T}_H/T$.\
\label{algo:1passal_line11}
\end{algorithm}

\begin{algorithm}

\caption{\rouone}\label{algo:sub1}

Set $\cF_1 \leftarrow \emptyset$. Initiate an (unweighted) reservoir sampler $\mbox{{\sc RS}}$  to store (up to) $\tOh(m/\sqrt{T})$ edges.\
\label{algo:1passalsub1_line1}

Note that $\cF_1$ is the set of edges stored by {\sc RS}.

\For{every vertex $u$ when its adjacency list is revealed}{
Perform the following steps in parallel:

{\bf Step 1:} \label{algo:1passalsub1_line2}
\For{every edge $e=(u,v)$}{

\uIf{$(v,u) \in \cF_1$}{
 Set $flag(e)=1$. \label{algo:1passalsub1_line3}
 
}

Give $e=(u,v)$ as an input to ${\sc RS}$.\ \label{algo:1passalsub1_line4}
}
%\label{algo:1passalsub1_line5}
{\bf Step 2:} \For{every edge $e=(v,w) \in \cF_1$}{ \label{algo:1passalsub1_line5}

\uIf{$flag(e)=0$ and $u$ forms a triangle $\Delta$ with $e$}{

$t_{e} \leftarrow t_{e} + 1$.\ \label{algo:1passalsub1_line6}

Give $\Delta$ as input to {\sc RS} that samples a triangle charged to $e$ uniformly at random. \label{algo:1passalsub1_line7}

} 

}

Let $\cF_1$ and $\cF'_1$ be the set of sampled edges by $\mbox{{\sc RS}}$ before and after the adjacency list of $u$ has been revealed, respectively.

\For{every edge $e \in \cF_1 \setminus \cF'_1$}{

Delete all information corresponding to $e$.\ \label{algo:1passalsub1_line8}
}

\For{every edge $e \in \cF'_1 \setminus \cF_1$}{

Set $flag(e)=0$ and initiate an (unweighted) reservoir sampler to sample a triangle charged on $e$ uniformly at random. \label{algo:1passalsub1_line9}

}
% \remove{
% {\bf Process (at the end of the stream):}

% Set $\tau \leftarrow \left(\frac{1+\eps/10}{1-\eps/10}\right)\sqrt{T/\eps}$.

% \uIf{$flag(e_s)=1$ and $0<t_{e_s} \leq \tau$}
% {
% Report $\Delta_s$ with probability $\frac{t_{e_s}}{\tau}$. With remaining probability, Return {\sc Fail}.\
% }

%   \uElse{
      
%       Return {\sc Fail}.
%    }   }
}



\end{algorithm}

\begin{algorithm}
\caption{\routwo}\label{algo:sub2}
Set $\cF_2 \leftarrow \emptyset$, and $\kappa=10\log n$.\ \label{algo:1passalsub2_line1}

%Set $\kappa=\left(1-\frac{\eps}{10}\right) \frac{ \tau \log n}{\sqrt{T}}$.\

Initialize a weighted reservoir sampler {\sc WRS}.\ \label{algo:1passalsub2_line2}

\For{every vertex $u$ when its adjacency list is revealed}
{

Perform the following steps in parallel:

{\bf Step 1:} \For{every edge $e=(u,v)$ in the stream}
{\label{algo:1passalsub2_line3}
Set $x_e=0$. \label{algo:1passalsub2_line4}

If {$e \in \cF_2$}, 
Set $flag(e)=1$.\ \label{algo:1passalsub2_line5}



\uElse{

Set $flag(e)=0$.\ \label{algo:1passalsub2_line6}

}

Sample $(u,v)$ with probability $p= \log n/\eps^2 \sqrt{T}$.\ \label{algo:1passalsub2_line7}

$\cF_2 \leftarrow \cF_2 \cup (u,v)$.\ \label{algo:1passalsub2_line8}

}
%\label{algo:1passalsub2_line9}
{\bf Step 2:} \For{each edge $e = (x,w) \in \cF_2$ such that $flag(e)=1$}{ 

\label{algo:1passalsub2_line9}

Determine if $(u,x,w)$ is a triangle.\ \label{algo:1passalsub2_line10}

$x_{e}\leftarrow x_{e}+1$. \label{algo:1passalsub2_line11}

}


{\bf Processing information obtained from Step 1 and 2:}

After the adjacency list of $u$ gets exposed, for each edge $e$ revealed during the exposure of $u$, do the following: 

\uIf{${x}_e \geq \kappa$}{

Give $({x_e},\Delta_e)$ as an input of {\sc WRS}, where $\Delta_e$ is a triangle taken uniformly at random among the set of triangles charged to $e$ and detected in Step 2.

}

\uIf{$x_e <\kappa$}{ 

Set $light(e)=1$.\ \label{algo:1passalsub2_line12}

}

$\widehat{t}_e=\frac{1}{p} \cdot x_e$.\ \label{algo:1passalsub2_line13}

$\widehat{T}_H \leftarrow  \widehat{T}_H + \widehat{t}_e$.\ \label{algo:1passalsub2_line14}

}

\end{algorithm}

\begin{algorithm}
\caption{{\sc Sample-Light-Triangle}}\label{alg:1passallight} 

%\begin{algorithmic}


\SetAlgoLined

%Set $\tau \leftarrow \left(\frac{1+\eps/10}{1-\eps/10}\right)\sqrt{T/\eps}$.
Set $\tau=900 \sqrt{T}, \mbox{{\sc Sampled-Triangle}} \leftarrow \emptyset$.\ \label{alg:1passallight_line1}

\For{every edge $e \in \cF_1$ with $flag(e)=1$ and $light(e)=1$}{
\label{alg:1passallight_line2}

With probability $\min\{{t_e}/{\tau},1\}$, keep the random triangle $\Delta_L$ charged to $e$ reported by corresponding reservoir sampler (if it exists).
\label{alg:1passallight_line3}

$\mbox{\sc Sampled-Triangle} \leftarrow \mbox{\sc Sampled-Triangle} \cup \Delta_L$.

} 

\uIf{$\mbox{{\sc Sampled-Triangle}} \neq \emptyset$}{ 

Report one triangle in {\sc Sampled-Triangle}  arbitrarily.\ \label{alg:1passallight_line4}
}

Otherwise, return {\sc Fail}. \label{alg:1passallight_line5}
 


%\end{algorithmic}

\end{algorithm}

\begin{algorithm}
\caption{{\sc Sample-Heavy-Triangle}}\label{alg:1passalheavy} 

\uIf{{\sc WRS} outputs $({x}_e,\Delta_e)$}{ 
\label{alg:1passalheavy_line1}

Report $\Delta_e$.\ \label{alg:1passalheavy_line2}

}

\uElse{

Report {\sc Fail}.\ \label{alg:1passalheavy_line3}

}

% \uIf{{\sc WRS} does not output anything}{

% Report {\sc Fail}.\

% }

% \uElse{

% $({x}_e,\Delta_e) \leftarrow {\sc WRS}$.\

% $\Delta_H \leftarrow \Delta_e$.\

% Report $\Delta_H$.\

% }
\end{algorithm}



==> algo_al_1_pass.tex <==
\section{Algorithm for AL 1 pass}
test
% \begin{minipage}{0.5\textwidth}
% \begin{algorithm}\label{algo:sub1}
% \caption{\rouone}
% \SetAlgoLined

% Set $\cF_1 \leftarrow \emptyset$. Initiate an (unweighted) reservoir sampler $\mbox{{\sc RS}}$  to store (up to) $\tOh(m/\sqrt{T})$ edges.\
% \label{algo:1passalsub1_line1}

% Note that $\cF_1$ is the set of edges stored by {\sc RS}.

% \For{every vertex $u$ when its adjacency list is revealed}{
% Perform the following steps in parallel:

% {\bf Step 1:} \label{algo:1passalsub1_line2}
% \For{every edge $e=(u,v)$}{

% \uIf{$(v,u) \in \cF_1$}{
%  Set $flag(e)=1$. \label{algo:1passalsub1_line3}
 
% }

% Give $e=(u,v)$ as an input to ${\sc RS}$.\ \label{algo:1passalsub1_line4}
% }
% %\label{algo:1passalsub1_line5}
% {\bf Step 2:} \For{every edge $e=(v,w) \in \cF_1$}{ \label{algo:1passalsub1_line5}

% \uIf{$flag(e)=0$ and $u$ forms a triangle $\Delta$ with $e$}{

% $t_{e} \leftarrow t_{e} + 1$.\ \label{algo:1passalsub1_line6}

% Give $\Delta$ as input to {\sc RS} that samples a triangle charged to $e$ uniformly at random. \label{algo:1passalsub1_line7}

% } 

% }

% Let $\cF_1$ and $\cF'_1$ be the set of sampled edges by $\mbox{{\sc RS}}$ before and after the adjacency list of $u$ has been revealed, respectively.

% \For{every edge $e \in \cF_1 \setminus \cF'_1$}{

% Delete all information corresponding to $e$.\ \label{algo:1passalsub1_line8}
% }

% \For{every edge $e \in \cF'_1 \setminus \cF_1$}{

% Set $flag(e)=0$ and initiate an (unweighted) reservoir sampler to sample a triangle charged on $e$ uniformly at random. \label{algo:1passalsub1_line9}

% }
% \end{algorithm}
% \end{minipage}

\begin{minipage}{0.45\textwidth}
\small{
\begin{algorithm}\label{alg:1passallight} 
\caption{{\sc Sample-Light-Triangle}}
\SetAlgoLined
\SetKw{Continue}{continue}

%Set $\tau \leftarrow \left(\frac{1+\eps/10}{1-\eps/10}\right)\sqrt{T/\eps}$.

Set $\tau=900 \sqrt{T}, \mbox{{\sc Sampled-Triangle}} \leftarrow \emptyset$.\ \label{alg:1passallight_line1}

\For{every edge $e \in \cF_1$ with $flag(e)=1$ and $light(e)=1$}{
\label{alg:1passallight_line2}

With probability $\min\{{t_e}/{\tau},1\}$, keep the random triangle $\Delta_L$ charged to $e$ reported by corresponding reservoir sampler (if it exists).
\label{alg:1passallight_line3}

$\mbox{\sc Sampled-Triangle} \leftarrow \mbox{\sc Sampled-Triangle} \cup \Delta_L$.

} 

\uIf{$\mbox{{\sc Sampled-Triangle}} \neq \emptyset$}{ 

Report one triangle in {\sc Sampled-Triangle}  arbitrarily.\ \label{alg:1passallight_line4}
}

Otherwise, return {\sc Fail}. \label{alg:1passallight_line5}
 


%\end{algorithmic}

\end{algorithm}
}
\end{minipage}
\hfill
\begin{minipage}{0.5\textwidth}
\begin{algorithm}\label{alg:1passalheavy}
\caption{{\sc Sample-Heavy-Triangle}}\ 

\uIf{{\sc WRS} outputs $({x}_e,\Delta_e)$}{ 
\label{alg:1passalheavy_line1}

Report $\Delta_e$.\ \label{alg:1passalheavy_line2}

}

\uElse{

Report {\sc Fail}.\ \label{alg:1passalheavy_line3}

}

% \uIf{{\sc WRS} does not output anything}{

% Report {\sc Fail}.\

% }

% \uElse{

% $({x}_e,\Delta_e) \leftarrow {\sc WRS}$.\

% $\Delta_H \leftarrow \Delta_e$.\

% Report $\Delta_H$.\

% }
\end{algorithm}
\end{minipage}

% \begin{minipage}{0.4\textwidth}
% \begin{algorithm}
% \caption{\routwo}\label{algo:sub2}
% Set $\cF_2 \leftarrow \emptyset$, and $\kappa=10\log n$.\ \label{algo:1passalsub2_line1}

% %Set $\kappa=\left(1-\frac{\eps}{10}\right) \frac{ \tau \log n}{\sqrt{T}}$.\

% Initialize a weighted reservoir sampler {\sc WRS}.\ \label{algo:1passalsub2_line2}

% \For{every vertex $u$ when its adjacency list is revealed}
% {

% Perform the following steps in parallel:

% {\bf Step 1:} \For{every edge $e=(u,v)$ in the stream}
% {\label{algo:1passalsub2_line3}
% Set $x_e=0$. \label{algo:1passalsub2_line4}

% If {$e \in \cF_2$}, 
% Set $flag(e)=1$.\ \label{algo:1passalsub2_line5}



% \uElse{

% Set $flag(e)=0$.\ \label{algo:1passalsub2_line6}

% }

% Sample $(u,v)$ with probability $p= \log n/\eps^2 \sqrt{T}$.\ \label{algo:1passalsub2_line7}

% $\cF_2 \leftarrow \cF_2 \cup (u,v)$.\ \label{algo:1passalsub2_line8}

% }
% %\label{algo:1passalsub2_line9}
% {\bf Step 2:} \For{each edge $e = (x,w) \in \cF_2$ such that $flag(e)=1$}{ 

% \label{algo:1passalsub2_line9}

% Determine if $(u,x,w)$ is a triangle.\ \label{algo:1passalsub2_line10}

% $x_{e}\leftarrow x_{e}+1$. \label{algo:1passalsub2_line11}

% }


% {\bf  After gathering information from Step 1 and 2:}

% After the adjacency list of of $u$ gets exposed, for each edge $e$ revealed during the exposure of $u$ such that 

% \uIf{${x}_e \geq \kappa$}{

% Give $({x_e},\Delta_e)$ as an input of {\sc WRS}, where $\Delta_e$ is a triangle taken uniformly at random among the set of triangles charged to $e$ and detected in Step 2.

% }

% \uIf{$x_e <\kappa$}{ 

% Set $light(e)=1$.\ \label{algo:1passalsub2_line12}

% }

% $\widehat{t}_e=\frac{1}{p} \cdot x_e$.\ \label{algo:1passalsub2_line13}

% $\widehat{T}_H \leftarrow  \widehat{T}_H + \widehat{t}_e$.\ \label{algo:1passalsub2_line14}

% }
% \end{algorithm}
% \end{minipage}

==> ea_temp.tex <==
\subsubsection{$2$-pass Triangle Sampling Algorithm in \ea/\va Model using $\Oh(\frac{m}{\sqrt{T}})$ Space}

We begin with the following claim, which roughly states that the samples $\cS$ and $\cF$ taken in Pass $1$ correctly decides whether the vertex (edge) $\Lambda$ is $\tau$-heavy or not.

\begin{cl}
    \begin{itemize}
        \item[(i)] If a vertex $v$ is $\tau$-light in $G$, then Algorithm~\ref{alg:2passea1} decides it correctly in the processing step with high probability.

        \item[(ii)] If an edge $e$ is $\tau$-light in $G$, then Algorithm~\ref{alg:2passea1} decides it correctly in the processing step with high probability.
    \end{itemize}
\end{cl}

\begin{lem}
    Algorithm~\ref{alg:2passea1} samples a light triangle uniformly using constant space with high probability.
\end{lem}


\begin{algorithm}
\caption{Triangle Sampling in $2$-pass \ea/\va Model}
\label{alg:2passea1}

\begin{algorithmic}
\State {\bf Pass 1}: Take $\Oh(\frac{n}{\sqrt{T}})$ many vertices $\cS$ and a set $\cF$ of $\Oh(\frac{m}{\sqrt{T}})$ many edges uniformly and independently at random with replacement~\footnote{Note that in the stream, only edges of the graph will appear. We use an $\ell_0$-sampler to sample the set of vertices $S$.}.

\

\State {\bf Pass 2}:
Select a vertex or an edge from the stream $\cM$ uniformly at random. Let $\Lambda$ be the selected element.

%\State {\bf Pass 3:} For each edge $e = \{a,b\} \in M$, do the following:
%Order the set $S$ and  $F$ randomly.

\

\State {\bf Process}:

\State Set $\tau \leftarrow \sqrt{\frac{T}{\eps}}$

\If{$\Lambda$ is a vertex}

\State Test if $\Lambda$ is $\tau$-light using $\cS$ and $\cF$ sampled in Pass $1$.

\If{($\Lambda$ is $\tau$-heavy)} 
   \State {\sc Ignore} $\Lambda$.

\Else

\State {\sc Report} a uniformly sampled triangle $\Delta$ with $\Lambda$ as a vertex with probability $\frac{t_{\Lambda}}{\tau}$.

\EndIf

\EndIf

\If{$\Lambda$ is an edge}

\State Test if $\Lambda$ is $\tau$-light using $\cS$ and $\cF$ sampled in Pass $1$.

\If{($\Lambda$ is $\tau$-heavy)} 
   \State {\sc Ignore} $\Lambda$.

\Else

\State {\sc Report} a uniformly sampled triangle $\Delta$ with $\Lambda$ as an edge with probability $\frac{t_{\Lambda}}{\tau}$.

\EndIf

\EndIf
\end{algorithmic}
\end{algorithm}

Finally, we will run Algorithm~\ref{alg:2passea1} ?? many times, and output an arbitrary triangle among the set of triangles sampled during the various invocations of the algorithm.


% \begin{algorithm}
% \caption{$2$-pass-\ea-model}\label{alg:2passea}

% \begin{algorithmic}
% \State {\bf Pass 1}: Take $\Oh(\frac{n}{\sqrt{T}})$ many vertices $S$ and a set $F$ of $\Oh(\frac{m}{\sqrt{T}})$ many edges uniformly and independently at random with replacement.
% Then find the set of all neighbors $N(S)$ of the set $S$.
% \State {\bf Pass 2}: Store all the edges of the induced graph $G[N(S)]$.

% %\State {\bf Pass 3:} For each edge $e = \{a,b\} \in M$, do the following:
% Order the set $S$ and  $F$ randomly.
% \State {\bf Process}:
% \For{(each $s \in S$)}
% \State Find $T_s$ and set $t_s = \size{T_s}$// This is possible as we have $G[N[S]]$ with us

% \State  If $t_S\neq 0$, then sample a triangle $\{s,a,b\}$ in $T_s$
% \EndFor

% \For{(each $e \in X$)}

% \State Find $T_e^S$ and set $t_e^S = \size{T_e^S}$ // This is possible as we have $G[N[S]]$ with us
% \State  If $t_e^S \neq 0$, then sample a triangle $\{s,a,b\}$ 

% \EndFor

% \State Call EdgeWeight($e, G[N(S)]$).
% \If{$e$ is {\sc Heavy}} 
%     \State {\sc Report} {\sc Fail}.
% \Else
% \State Consider the multi-set of triangles $T(e,S)$ that $e$ forms with $S$. Sample one triangle $t_1 = \{a,b,s\}$ uniformly at random from $T(e,S)$.
% \State Call VertexWeight($s, G[N(S)]$).
%     \If{$s$ is {\sc Heavy}}
%         \State {\sc Report} $t_1$.
%     \Else
%          \State {\sc Report} $t_1$ with probability $\frac{1}{2}$.
%     \EndIf
% \EndIf 
% \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}
% \caption{EdgeWeight(e, G[N(S)])}\label{alg:edgeweight}
% \begin{algorithmic}
% \If{$t(e,S) \geq \frac{50 \log n}{\eps^2}$} 
%     \State {\sc Report} {\sc Heavy}.
% \Else
%      \State {\sc Report} {\sc light}.
% \EndIf 
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}
% \caption{VertexWeight(s, G[N(S)])}\label{alg:edgeweight}
% \begin{algorithmic}
% \If{$t^c_s > 100 \sqrt{\frac{T}{\eps}}$} 
%     \State {\sc Report} {\sc Heavy}.
% \Else
%      \State {\sc Report} {\sc light}.
% \EndIf 
% \end{algorithmic}
% \end{algorithm}

==> lower_bound.tex <==
\section{Lower Bound Results for Triangle Sampling}\label{sec:lb}

Let us start this section by recalling a result regarding estimating the bias of a coin.

\begin{obs}[Folklore]\label{obs:estbias}
Let us assume $C$ be a coin such that the probability of appearing head of $C$ is $p$. Then we have the following:
\begin{enumerate}
    \item[(i)] To obtain an estimate $\widehat{p}$ of $p$ such that $|p-\widehat{p}| \leq \eps p$, $\Theta(1/p \eps^2)$ tosses of $C$ are necessary and sufficient. 

    \item[(ii)] To obtain an estimate $\widehat{p}$ of $p$ such that $|p-\widehat{p}| \leq \eps $, $\Theta(1/\eps^2)$ tosses of $C$ are necessary and sufficient.
\end{enumerate}
\end{obs}

Let us construct an algorithm for obtaining a multiplicative estimate of the number of triangles present in the underlying graph $G$ by using an algorithm that samples a triangle of $G$ uniformly. 

\begin{obs}[Sampling to Counting reduction]\label{obs:samplingcountingreduction}
    Any triangle sampling algorithm that samples a triangle either uniformly or in at most $\eps$ $\ell_1$-distance from a graph $G$ can be converted to a triangle counting algorithm, that provides a $(1 \pm \eps)$-multiplicative estimate of the number of triangles of $G$, where $\eps \in (0,1)$ is a proximity parameter.
    Moreover, the space complexity of the triangle counting algorithm is in similar order of that of triangle sampling algorithm, ignoring polynomial dependence on $1/\eps$.   
    %can be used to design a triangle counting algorithm, that provides a $(1 \pm \eps)$-multiplicative estimate of the number of triangles present in the underlying graph $G$, where $\eps \in (0,1)$ is a proximity parameter.
\end{obs}

\begin{proof}
We will argue below for the case of a sampling algorithm that samples triangles uniformly from $G$. Similar arguments hold for the case when the algorithm samples triangles following a distribution that has $\ell_1$-distance at most $\eps$ from the uniform distribution.

Let $\cA$ be an algorithm that samples a triangle from $G$ uniformly. The success probability $p$ of $\cA$ depends upon the number of triangles present in the underlying graph $G$. Using Observation~\ref{obs:estbias}, we can say that the total number of triangles in $G$ can be estimated within $(1 \pm \eps)$-factor by applying $\cA$ $\Theta(1/p\eps^2)$ times. This implies that we can count the number of triangles by applying the triangle sampling algorithm $\cA$ $\Theta(1/p\eps^2)$ times. 

Thus any lower bound for the triangle counting algorithm will directly provide us with a lower bound of the triangle sampling algorithm, ignoring the dependency on the proximity parameter $\eps$. Finally, by the design of the triangle counting algorithm, it is clear that the space complexity of the counting algorithm remains in a similar order as the sampling algorithm, ignoring the dependencies on $1/\eps$. This completes the proof of the observation.
\end{proof}





Due to a shortage of space, the proof of this observation is presented in Appendix~\ref{sec:lb_app}. Now we will state our lower bound results starting with \ea/\va model.

% \begin{proof}
% We will argue below for the case of a sampling algorithm that samples triangles uniformly from $G$. Similar arguments hold for the case when the algorithm samples triangles following a distribution that has $\ell_1$-distance at most $\eps$ from the uniform distribution.

% Let $\cA$ be an algorithm that samples a triangle from $G$ uniformly. The success probability $p$ of $\cA$ depends upon the number of triangles present in the underlying graph $G$. Using Observation~\ref{obs:estbias}, we can say that the total number of triangles in $G$ can be estimated within $(1 \pm \eps)$-factor by applying $\cA$ $\Theta(1/p\eps^2)$ times. This implies that we can count the number of triangles by applying the triangle sampling algorithm $\cA$ $\Theta(1/p\eps^2)$ times. 

% Thus any lower bound for triangle counting algorithm will directly provide us a lower bound of triangle sampling algorithm, ignoring the dependency on the proximity parameter $\eps$. Finally, by the design of the triangle counting algorithm , it is clear that the space complexity of the counting algorithm remains in similar order as the sampling algorithm, ignoring the dependencies on $1/\eps$. This completes the proof of the observation.
% \end{proof}

%Let us denote the success probability of $\cA$ by $p$, where $p \in (0,1)$ be a parameter that depends upon the number of triangles in $G$.

%Now let us consider a coin whose probability of head is $p$. Using concentration inequalities, we know that $\Theta(\frac{1}{p \eps^2})$ many tosses of the coin are necessary and sufficient to obtain a $(1 \pm \eps)$-multiplicative estimate $\hat{p}$ of $p$, where $\eps \in (0,1)$ is a proximity parameter.

\subsection{Lower bound for Triangle Sampling in \ea/\va Model}\label{sec:ealb}

% \begin{lem}[Lower bound for Triangle Counting in 1-pass, Theorem 1 of \cite{braverman2013hard}]
%     For any $m, T \in \N$ such that $T = \Omega(m)$, there exist $m' = \Theta(m)$ and $T'=\Theta(T)$ such that any \ea (\va) streaming algorithm that distinguishes between $m'$-edge graphs with $0$ and $T'$ triangles in $1$-pass with probability at least $2/3$ requires $\Omega(m^2/T)$ space.
% \end{lem}

%\comment{Sayantan: Check the reference and shall we write $\min\{m, m^2/T\}$?}

Following Observation~\ref{obs:samplingcountingreduction}, and triangle counting lower bound from ~\cite[Theorem 1]{braverman2013hard}, we have the following lower bound of triangle sampling in $1$ pass in \ea (\va) model.

\begin{theo}[Lower bound of Theorem~\ref{theo:ea1pass}]
    For any $m, T \in \N$ such that $T = \Omega(m)$, there exist $m' = \Theta(m)$ and $T'=\Theta(T)$ such that any \ea (\va) streaming algorithm that samples a triangle from a graph with $m'$ edges and $T'$ triangles in $1$-pass with probability at least $2/3$ requires $\Omega(m^2/T)$ space.
\end{theo}



% \begin{lem}[Lower bound for Triangle Counting in Multi-pass, Theorem 4.2 of \cite{bera2017towards}]
%     For any $m, T \in \N$ such that $T = \Omega(m)$, there exist $m' = \Theta(m)$ and $T'=\Theta(T)$ such that any \ea (\va) streaming algorithm that distinguishes between $m'$-edge graphs with $0$ and $T'$ triangles in multi-pass with probability at least $2/3$ requires $\Omega(m^{3/2}/T)$ space.
% \end{lem}

Similar to above, we have the following multi-pass lower bound for triangle sampling from ~\cite[Theorem 4.2]{bera2017towards} and Observation~\ref{obs:samplingcountingreduction}.


\begin{theo}[Lower bound of Theorem~\ref{theo:ea3pass}]
    For any $m, T \in \N$ such that $T = \Omega(m)$, there exist $m' = \Theta(m)$ and $T'=\Theta(T)$ such that any \ea (\va) streaming algorithm samples a triangle from any graph with $m'$ edges and $T'$ triangles in multi-pass with probability at least $2/3$ requires $\Omega(m^{3/2}/T)$ space.
\end{theo}

\subsection{Lower bound for Triangle Sampling in \al Model}\label{sec:allb}


% \begin{lem}[Lower bound for Triangle Counting in 1-pass, Theorem 5.1 of \cite{kallaugher2019complexity}]
% For any $m, T \in \N$ such that $T \leq m$, there exist $m' = \Theta(m)$ and $T'=
% \Theta(T)$ such that any \al streaming algorithm that distinguishes between $m'$-edge graphs with $0$ and $T'$ triangles in one pass with probability at least $2/3$ requires $\Omega(m/\sqrt{T})$ space.
% \end{lem}

Similar to \ea/\va model, we have the following $1$-pass lower bound for triangle sampling from ~\cite[Theorem 5.1]{kallaugher2019complexity}.

\begin{theo}[Lower bound of Theorem~\ref{theo:al1pass}]
For any $m, T \in \N$ such that $T \leq m$, there exist $m' = \Theta(m)$ and $T'=
\Theta(T)$ such that any \al streaming algorithm that samples a triangle uniformly from any graph with $m'$ edges and $T'$ triangles in one pass with probability at least $2/3$ requires $\Omega(m/\sqrt{T})$ space.
\end{theo}

% \begin{lem}[Lower bound of Triangle Counting in Multi-pass, Theorem 5.2 of \cite{kallaugher2019complexity}]
% For any $m,T \in \N$ such that $T \leq m^{3/2}$, there exist $m'= \Theta(m)$ and $T'=\Theta(T)$ such that any adjacency list streaming algorithm that
% distinguishes between $m'$-edge graphs with $0$ and $T'$ triangles with probability at least $2/3$ in a constant number of passes requires $\Omega(m/T^{2/3})$ space.
% \end{lem}

Finally, we have our multi-pass lower bound of triangle sampling from Observation~\ref{obs:samplingcountingreduction}, and triangle counting lower bound from ~\cite[Theorem 5.2]{kallaugher2019complexity}.

\begin{theo}[Lower bound of Theorem~\ref{theo:al3pass}]
For any $m,T \in \N$ such that $T \leq m^{3/2}$, there exist $m'= \Theta(m)$ and $T'=\Theta(T)$ such that any adjacency list streaming algorithm that samples a triangle uniformly from any graph with $m'$ edges and $T'$ triangles with probability at least $2/3$ in a constant number of passes requires $\Omega(m/T^{2/3})$ space.
\end{theo}


%\comments{Sayantan: To check}


==> proof_al_app.tex <==
\section{Remaining Proofs from Section~\ref{sec:alub}}\label{sec:al_app}


We will use the following result which upper bounds the maximum number of triangles of a graph $G$ with respect to its number of edges which will be used in our proof.

\begin{lem}[\cite{RIVIN2002647}]\label{lem:boundnumbertriangle}
    Given a graph $G(V,E)$ such that $\size{E}=m$, the maximum number of triangles of $G$ is at most $\Oh(m^{3/2})$.
\end{lem}


\begin{obs}[Restatement of Observation~\ref{obs:al3passboundno}]\label{obs:al3passboundno_app}
Let us assume that in a graph $G$, the total number of triangles is $T$ and $\tau=12(T/\eps^2)^{1/3}$ is an integer. Then we have the following:
\begin{description}
    \item[(i)] Number of $\tau$-heavy edges is at most $ (\eps T/8)^{2/3}$.
    
    \item[(ii)] Number of heavy triangles $T_H$ is at most $\eps T/8$.
    
    \item[(iii)] Number of light triangles $T_L$ is at least $(1-\eps /8 )T$.
\end{description}
\end{obs}

\begin{proof}

\begin{description}

\item[(i)] From the definition of $\tau$-heavy edges (Definition~\ref{defi:heavylightedge}), an edge $e$ is $\tau$-heavy, if the number of triangles $t_e$ incident on $e$ is at least $\tau$. Since the total number of triangles in the graph $G$ is $T$, the total number of $\tau$-heavy edges can be at most $3T/\tau$. As $\tau = 12(T/\eps^2)^{1/3}$, the result follows.

\item[(ii)] Following the result regarding bounding the total number of triangles in a graph with respect to its number of edges (Lemma~\ref{lem:boundnumbertriangle}), we know that the total number of possible triangles over $m$ edges is at most $\Oh(m^{3/2})$. Since from $(i)$, we know that the total number of $\tau$-heavy edges is at most $\mathcal{O}((\eps T /8 )^{2/3})$, we have the result.

\item[(iii)] Follows directly from $(ii)$ as $T=T_L+T_H$.
\end{description}
\end{proof}



==> proof_ea_app.tex <==
\section{Remaining Proofs from Section~\ref{sec:eaalgo}}\label{sec:ea_app}

\begin{theo}[Restatement of Theorem~\ref{theo:tsamp-arb-1-proof}]\label{theo:tsamp-arb-1-proof_app}
\tsamp can be solved by using $\tOh\left(\min\{m,m^{2}/T\}\right)$ space in \ea/\va model in $1$-pass.
\end{theo}

\begin{proof}[Proof of Theorem~\ref{theo:tsamp-arb-1-proof}]

First we argue about space complexity.

\paragraph*{Space Complexity:}
%Let us first start by arguing the space complexity of the algorithm corresponding to Theorem~\ref{theo:tsamp-arb-1-proof}. From the description, it is clear that

Algorithm~\ref{alg:1passea} uses only two sets as variables: $\mbox{{\sc Edge-Set}}$ and $\mbox{{\sc Triangle-Sampled}}$ which store $\Oh(1)$ edges in a single invocation of Algorithm~\ref{alg:1passea}. Since we run $\tOh(m^2/T)$ instances of Algorithm~\ref{alg:1passea} in parallel, the total space complexity is $\tOh(m^2/T)$.

%So Algorithm~\ref{alg:1passea} uses only constant space during its single execution.

\paragraph*{Proof of Correctness:}
%Let us now proceed with the correctness proof of Algorithm~\ref{alg:1passea}. 

% \begin{lem}\label{lem:eaalgo1}
% Algorithm~\ref{alg:1passea} samples a triangle of $G$ uniformly. Moreover, the amount of space used by Algorithm~\ref{alg:1passea} is constant.
% \end{lem}

% \begin{proof}
%First note that Algorithm~\ref{alg:1passea} uses only two sets as variables: $\mbox{{\sc Edge-Set}}$, $\mbox{{\sc Triangle-Sampled}}$ which stores constant number of edges in a single invocation of Algorithm~\ref{alg:1passea}. Thus, it is immediate that Algorithm~\ref{alg:1passea} uses constant space during its execution.

To prove that Algorithm~\ref{alg:1passea} samples a triangle uniformly, let us consider an arbitrary triangle $\Delta= (e_1, e_2, e_3)$, and define the following two events $E_1$ and $E_2$:
\begin{center}
$E_1$:= Edges $e_1$ \mbox{and} $e_2$ stored in Line~\ref{algo:1passea_line1} have not been replaced by other edges till the algorithm terminates.

$E_2$:= Algorithm~\ref{alg:1passea} outputs a sampled triangle.
\end{center}
First note that if the edges $e_1$ and $e_2$ have not been replaced during the execution of Algorithm~\ref{alg:1passea}, then when the edge $e_3$ appears in the stream, the triangle $\Delta$ will be sampled.
Thus, the probability that $\Delta$ has been sampled is: $\pr(E_1) = 1/m^2$.

% \begin{eqnarray*}
% \pr(\Delta \ \mbox{has been sampled}) &=& \pr(E_1) = \frac{1}{m^2}
% \end{eqnarray*}

%$$E_1:= \Delta \ \mbox{has been sampled by Algorithm~\ref{alg:1passea}}$$
% Let us now define another random variable $E_3$ as follows:
% $$E_3:= \mbox{Algorithm~\ref{alg:1passea} outputs a sampled triangle}$$

Since there are $T$ triangles in the graph $G$ and the triangles reported by the algorithm are disjoint event, using the union bound, we can say that the probability that Algorithm~\ref{alg:1passea} outputs a sampled triangle is: $\pr(E_2) = T/m^2$.

Since we are running $t= \tOh(m^2/T)$ instances of Algorithm~\ref{alg:1passea} in parallel, the probability that no triangle will be sampled among all the instances is bounded by $(1 - T/m^2)^{t} \leq 1/poly(n)$. Thus, we conclude that with probability at least $1- 1/poly(n)$, a triangle will be sampled.


%As reporting distinct triangles are disjoint events, using the union bound over all possible $T$ triangles of the graph $G$, we can say that the probability that Algorithm~\ref{alg:1passea} outputs a sampled triangle is: $\pr(E_2) = \frac{T}{m^2}$.

%So, the probability that any triangle has been sampled is $\frac{T}{m^2}$.

Now we will argue that Algorithm~\ref{alg:1passea} samples the triangle uniformly among all the triangles present in the graph. For this purpose, let us work on the conditional space that Algorithm~\ref{alg:1passea} has sampled a triangle. The probability that Algorithm~\ref{alg:1passea} has sampled $\Delta$ is same as the probability that the event $E_1$ occurs, given that the event $E_2$ holds, that is,
$\pr(E_1 \mid E_2) = \frac{\pr(E_1 \cap E_2)}{\pr(E_2)} = \frac{1/m^2}{T/m^2} = 1/T$.


% \begin{eqnarray*}
% \pr(E_1 \mid E_2) = \frac{\pr(E_1 \cap E_2)}{\pr(E_2)} = \frac{\frac{1}{m^2}}{\frac{T}{m^2}} = \frac{1}{T}
% \end{eqnarray*}

Thus, each triangle is sampled uniformly by Algorithm~\ref{alg:1passea}. This concludes the proof of the theorem.
\end{proof}

\begin{theo}[Restatement of Theorem~\ref{theo:tsamp-arb-p-proof_proof}]\label{theo:tsamp-arb-p-proof_proof_app}
\tsamp can be solved in $\tOh\left(m^{3/2}/T\right)$ space in \ea/\va model in $3$-passes.
\end{theo}

\begin{proof}[Proof of Theorem~\ref{theo:tsamp-arb-p-proof}]

We start with the space complexity.

%of our algorithm corresponding to Theorem~\ref{theo:tsamp-arb-p-proof}.

% Let us begin with the following lemma.

% \begin{lem}\label{lem:multipasseaalgo2}
% Algorithm~\ref{alg:3passea2} samples a triangle of $G$ uniformly. Moreover, it uses constant space during its execution.

% %with probability at least $1 - \frac{1}{m^c}$.
% \end{lem}

\paragraph*{Space Complexity:}
As seen in Algorithm~\ref{alg:3passea2}, all the passes require $\Oh(1)$ space. Since we are running $\widetilde{\Oh}(m^{3/2}/T)$ instances of Algorithm~\ref{alg:3passea2} in parallel, the total space used is $\widetilde{\Oh}(m^{3/2}/T)$.

%Let us first argue about the space complexity of Algorithm~\ref{alg:3passea2}. Note that in \textbf{Pass 1} and \textbf{Pass 2}, the algorithm samples two edges $(u,v)$ and $(x,y)$, and stores the degrees of the endpoints of the sampled edges, as well as a random neighbor of $u$ and $v$. Finally, in \textbf{Pass 3}, it checks two conditions, and decides about outputting the triangle $(u,v,w)$ based upon the outcomes of the conditions checked. Thus, Algorithm~\ref{alg:3passea2} uses constant space in a single execution.

%Since we are finally running $\tOh(\frac{m^{\frac{3}{2}}}{T})$ instances of Algorithm~\ref{alg:3passea2} in parallel, we conclude that $\tOh(\frac{m^{\frac{3}{2}}}{T})$ space is used in total.

\paragraph*{Proof of Correctness:}

Let us consider an arbitrary triangle $\Delta = (u,v,w)$. Note that $\Delta$ has been sampled by Algorithm~\ref{alg:3passea2} only if the edge $(u,v)$ has been sampled in Pass 1, as well as $w$ has been chosen in Pass 2. Thus the probability that $\Delta$ has been sampled by Algorithm~\ref{alg:3passea2} can be written as follows:
\begin{equation}\label{eqn:probdelsampled}
\begin{aligned}
    \pr(\Delta \ \mbox{has been sampled}) = \pr((u,v) \ \mbox{has been sampled in Pass 1}) \\ \times \ \pr(w \ \mbox{has been chosen in Pass 2}).
\end{aligned}    
\end{equation}

Now let us compute the second term in Equation~\ref{eqn:probdelsampled}. We consider the following two cases depending upon the degree of the vertex $u$.
\noindent
\paragraph*{\textbf{Case 1: $\deg(u) \leq \sqrt{2m}$:}} 
Note that the algorithm finds a random neighbor $u'$ of $u$ in Pass 2 in Line~\ref{algo:3passea_line5}. Then in the Process step, if $\deg(u) \leq \sqrt{2m}$, it proceeds with probability $\deg(u)/\sqrt{2m}$, and sets $w$ as $u'$. Since $u'$ has been chosen randomly among all the neighbors of $u$, the vertex $w$ is sampled with probability $1/\sqrt{2m}$.
\noindent
\paragraph*{\textbf{Case 2: $\deg(u) > \sqrt{2m}$:}}
When $\deg(u) > \sqrt{2m}$, the vertex $w$ is chosen uniformly among the vertices $\{x,y\}$ with equal probability. In that case, the probability that $w$ is sampled is as follows:
$$\pr(w \in \{x,y\}) \times \frac{1}{2} \times \frac{\sqrt{2m}}{\deg(w)} = \frac{\deg(w)}{m} \times \frac{1}{2} \times \frac{\sqrt{2m}}{\deg(w)} = \frac{1}{\sqrt{2m}}.$$


% \begin{description}
% \item[Case 1: $\deg(u) \leq \sqrt{2m}$:] 
% Note that the algorithm finds a random neighbor $u'$ of $u$ in Pass 2 in Line~\ref{algo:3passea_line4}. Then in the Process step, if $\deg(u) \leq \sqrt{2m}$, it proceeds with probability $\deg(u)/\sqrt{2m}$, and sets $w$ as $u'$. Since $u'$ has been chosen randomly among all the neighbors of $u$, the vertex $w$ is sampled with probability $1/\sqrt{2m}$.

% \item[Case 2: $\deg(u) > \sqrt{2m}$:]
% When $\deg(u) > \sqrt{2m}$, the vertex $w$ is chosen uniformly among the vertices $\{x,y\}$ with equal probability. In that case, the probability that $w$ is sampled is as follows:
% $$\pr(w \in \{x,y\}) \times \frac{1}{2} \times \frac{\sqrt{2m}}{\deg(w)} = \frac{\deg(w)}{m} \times \frac{1}{2} \times \frac{\sqrt{2m}}{\deg(w)} = \frac{1}{\sqrt{2m}}.$$

% \end{description}

Since the edges $\{u,v\}$ and $\{x,y\}$ are sampled uniformly in Pass 1, following Equation~\ref{eqn:probdelsampled}, we can say that the probability that the triangle $\Delta$ has been sampled is:
$(1/m) \times (1/\sqrt{2m}) = 1/\sqrt{2}m^{\frac{3}{2}}.$

Note that till now we have been arguing for a fixed triangle $\Delta$. Using the union bound over the $T$ triangles of $G$, we conclude that the probability that any triangle has been sampled by Algorithm~\ref{alg:3passea2} in a single execution is $T/\sqrt{2}m^{\frac{3}{2}}$.

Since we are running $t=\tOh(m^{\frac{3}{2}}/T)$ instances of Algorithm~\ref{alg:3passea2} in parallel, the probability that no triangle has been sampled is at most $(1- T/\sqrt{2}m^{\frac{3}{2}})^{t} \leq 1/poly(n)$.

Now let us prove that Algorithm~\ref{alg:3passea2} has sampled a triangle uniformly among all the triangles of the graph $G$. So, let us now work on the conditional space that a triangle has been sampled by Algorithm~\ref{alg:3passea2}. Under this conditional space, the probability that the particular triangle $\Delta$ has been sampled is:
\begin{eqnarray*}
    \pr\left(\frac{\Delta \ \mbox{has been sampled}}{ \mbox{A triangle has been sampled}}\right) = \frac{\frac{1}{\sqrt{2}m^{\frac{3}{2}}}}{\frac{T}{\sqrt{2}m^{\frac{3}{2}}}} = \frac{1}{T}
\end{eqnarray*}

Thus the triangle $\Delta$ has been sampled uniformly by Algorithm~\ref{alg:3passea2}. This completes the proof of Theorem~\ref{theo:tsamp-arb-p-proof}.
\end{proof}



==> temp.tex <==
{
\begin{algorithm}
\caption{{\sc Sample-Heavy-Triangle}}\label{alg:1passal} 
\remove{
\begin{algorithmic}
% \State Initialize two reservoir sampler $RS_1$ (for an edge sample) and $RS_2$ (for a triangle sample on the edge that is sampled).

\State Set $F := \emptyset$

\For{each vertex $u$ that is exposed}

\State Initialize $F'=\emptyset$

\For{each edge $e = \{u,v\}$ in the stream}
\uIf{(u,v) is temp-heavy}
\State Remove the flag that it is temp-heavy.

\EndIf

\If{$\{u,v\} \in F$}

\State $flag(e) \leftarrow 1$.

\Else

\State Sample $e = \{u,v\}$ with probability $\frac{10 \log n}{\sqrt{T}}$.

\If{$e$ is sampled}
\State Set $flag(e)=0$
\State $t_e=0$
\State Initialize a reservoir sampler for $e$.

\State $F':= F' \cup \{e\}$.

\EndIf

\State Store the information whether $(u,v)$ shares common vertices with edges in $F$, let us say the information to be $\cI$.
\EndIf

\EndFor

\For{each edge $e \in F$}

\If{$u$ and $e$ forms a triangle (can be decoded from $\cI$) and $flag(e)=0$}

\State $t_e \leftarrow t_e +1$.

\State Send the triangle containing $u$ and $e$ to the reservoir sampler $RS_2$ with respect to $e$.

\EndIf

\EndFor

\State Let $W \subseteq F$ such that the vertices for each $(x,y)\in W$, $(x,y)$ forms a triangle with $u$.

\If{$\size{W}\geq \log n$}

\State declare $\{u,v\}$ as \emph{temp-heavy}.

\State Sample an edge $(x,y)$ uniformly from $W$ and store the triangle $(x,y,u)$.

\EndIf

$F \leftarrow F \cup F'$

\EndFor

\State Consider the edges in $F'' \subset F$ such that for each $e \in F''$ either (i) $e$ is temp-heavy or (ii) $flag(e)=1$ and $t_e \geq \sqrt{T}$.


\State $\widehat{T_h}\leftarrow \sum\limits_{e \in F'': e~\mbox{is temp-heavy}} \sqrt{T}\cdot t_e + \sum\limits_{e \in F''} t_e $ 

\State Select $e \in F''$ with probability $\frac{t_e}{\widehat{T_h}}$ and output the triangle sampled corresponding to $e$.
\end{algorithmic}}
\end{algorithm}

Let us assume $F_1$ denotes a set of edges sampled from the stream $M$. Similarly assume that $F_2$ represents a multi-set of edges. For each edge $e$, store a counter $t_e$ that counts the number of triangles incident on $e$.
}
\begin{algorithm}
\caption{Triangle Sampling in 1 pass \al Model}\label{alg:1passal} 

\begin{algorithmic}



\end{algorithmic}
\end{algorithm}
